The $p$-arithmetic homology of mod $p$ representations of $\mathrm{GL}_2(\mathbb{Q}_p)$

We compute the non-Eisenstein systems of Hecke eigenvalues contributing to the $p$-arithmetic homology of irreducible smooth mod $p$ representations $\pi$ of $\mathrm{GL}_2(\mathbb{Q}_p)$ and to the cohomology of their duals. We show that in most cases they are associated to odd irreducible 2-dimensional Galois representations whose local component at $p$ corresponds under the mod $p$ local Langlands correspondence to a smooth representation that contains $\pi$ as a subrepresentation.

==> format_basic.tex <==
\makeatletter

\def\emptycleardoublepage{\clearpage\if@twoside \ifodd\c@page\else
\thispagestyle{empty}%
\hbox{}\newpage\if@twocolumn\hbox{}\newpage\fi\fi\fi}

\makeatother
\newenvironment{nscenter}
 {\parskip=0pt\par\nopagebreak\centering}
 {\par\noindent\ignorespacesafterend}
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\newtheoremstyle{note}%
{12pt}%
{9pt}%
{}%
{}%
{\bfseries}%
{.}%
{.5em}%
{}%
\newtheoremstyle{customnote}%
{12pt}%
{9pt}%
{}%
{}%
{\bfseries}%
{.}%
{.5em}%
{\def\temp{#3}\ifx\temp\empty\thmname{#1}\thmnumber{ #2}\else\thmnote{#3}\thmnumber{ #2}\fi}%
\newtheoremstyle{customnote*}%
{12pt}%
{9pt}%
{}%
{}%
{\bfseries}%
{.}%
{.5em}%
{\def\temp{#3}\ifx\temp\empty\thmname{#1}\else\thmnote{#3}\fi}%
\newtheoremstyle{thethm}%
{12pt}%
{3pt}%
{\itshape}%
{}%
{\bfseries}%
{.}%
{.5em}%
{}%
\theoremstyle{note}
\newtheorem{theorem}[equation]{Theorem}
\newtheorem*{theorem*}{Theorem}
\newreptheorem{theorem}{Theorem}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{claim}[equation]{Claim}
\newreptheorem{lemma}{Theorem}
\newtheorem{corollary}[equation]{Corollary}
\theoremstyle{note}
\newtheorem{remark}[equation]{Remark}
\newtheorem{fact}[equation]{Fact}
\newtheorem{example}[equation]{Example}
\newtheorem{notation}[equation]{Notation}
\newtheorem{exercise}[equation]{Exercise}
\newtheorem{prob}[equation]{Problem}
\newtheorem{definition}[equation]{Definition}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{question}[equation]{Question}
\newtheorem{question*}{Question}
\newtheorem{assumption}[equation]{Assumption}
\newtheorem{assumption*}{Assumption}
\newtheorem{construction}[equation]{Construction}
\theoremstyle{customnote}
\newtheorem{custom}[equation]{Theorem}
\theoremstyle{customnote*}
\newtheorem{custom*}{Theorem}
\renewenvironment{proof}[1][Proof]{\vspace{-0.3cm}\noindent\textit{#1. }}{\qed}
\numberwithin{equation}{section}
\setlength\parindent{6pt}
\setlength{\parskip}{0.5em}
\setlist[itemize]{topsep=0pt, leftmargin=6mm}
\setlist[enumerate]{topsep=0pt, label={\rm (\roman*)}}
\newcommand{\itemnumber}[1]{{\rm (\romannum{#1})}}
\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}
\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}
\def\showproofstwo{0}

